A Convergent and Dimension-Independent Min-Max Optimization Algorithm

We study a variant of a recently introduced min-max optimization framework where the max-player is constrained to update its parameters in a greedy manner until it reaches a first-order stationary point. Our equilibrium definition for this framework depends on a proposal distribution which the min-player uses to choose directions in which to update its parameters. We show that, given a smooth and bounded nonconvex-nonconcave objective function, access to any proposal distribution for the min-player's updates, and stochastic gradient oracle for the max-player, our algorithm converges to the aforementioned approximate local equilibrium in a number of iterations that does not depend on the dimension. The equilibrium point found by our algorithm depends on the proposal distribution, and when applying our algorithm to train GANs we choose the proposal distribution to be a distribution of stochastic gradients. We empirically evaluate our algorithm on challenging nonconvex-nonconcave test-functions and loss functions arising in GAN training. Our algorithm converges on these test functions and, when used to train GANs, trains stably on synthetic and real-world datasets and avoids mode collapse

==> images/strongly_convex_concave.tex <==

\newpage

\section{Equilibrium in the strongly convex-strongly concave setting}

\begin{assumption} \label{assumption_x_stochastic_gradient}$(\sigma)$
The distribution $Q_{x,y}$ satisfies $\mathbb{E}_{\Delta \sim Q_{x,y}}[\Delta] = \mu \nabla_x f(x,y)$ and $\mathbb{E}_{\Delta \sim Q_{x,y}}[\|\Delta -\frac{1}{L} \nabla_x\|^2] \leq \sigma^2$.
\end{assumption}

\begin{theorem}\label{thm_strongly_convex}
Suppose that $f: \mathbb{R}^d \times \mathbb{R}^d \rightarrow \mathbb{R}$ is $\alpha$-strongly convex in $x$ and $\alpha$-strongly concave in $y$, and $L$-smooth in both variables.
%
Then, for any $\eps, \delta, \omega>0$ and any proposal distribution $Q_{x,y}$ satisfying \eqref{assumption_x_stochastic_gradient} for some $\sigma\leq 0$, any point $(x^\star, y^\star)$ which is an $(\eps, \delta, \omega, Q)$-approximate local equilibrium of $f$ also has optimality gap satisfying
\begin{equation}
\max_{y \in \mathbb{R}^d} f(x^\star, y) -    \min_{x \in \mathbb{R}^d} f(x, y^\star) \leq =\frac{L\eps^2}{2\alpha^2} + 
    %
    \frac{L^3}{2\alpha^2}
   \left(\sqrt{\delta + L \left(2\frac{\eps}{\alpha} + \mu \frac{L}{\alpha}(L\frac{\eps}{\alpha} + \frac{\sigma}{\sqrt{\omega}})\right) + L \frac{\eps^2}{2 \alpha^2} +L \frac{\eps}{\alpha}} +  L \frac{\eps}{\alpha}\right)^2.
\end{equation}
\end{theorem}

\begin{remark}
In other words, Theorem \ref{thm_strongly_convex} says that, for any $\epsilon>0$ there are $\delta, \omega, \sigma = \mathrm{poly}(\frac{1}{L}, \frac{1}{\alpha}, \eps)$ independent of the dimension $d$,  such that any point $(x^\star, y^\star)$ which is an $(\eps, \delta, \omega, Q)$-approximate local equilibrium of $f$ also has optimality gap satisfying
%
\begin{equation}
\max_{y \in \mathbb{R}^d} f(x^\star, y) -    \min_{x \in \mathbb{R}^d} f(x, y^\star) \leq \eps.
\end{equation}

\end{remark}



In the following we set $\mu := \frac{1}{L}$.

\begin{lemma}\label{prop_strongly_convex_1}
For any $x, w \in \mathbb{R}^d$,
%
\begin{equation}
    \|\mathrm{argmax}_{z \in \mathbb{R}^d} f(x,z) -  \mathrm{argmax}_{z \in \mathbb{R}^d} f(\theta,z)\| \leq  \frac{L}{\alpha}\|\theta-x\|
\end{equation}
\end{lemma}

\begin{proof}
Since $f(x,\cdot)$ is concave, we have that a point $z$ is a global maximum if and only if $\nabla_y f(x,z) = 0$. 
%
Since $f(x,\cdot)$ is $\alpha$-strongly concave for $\alpha>0$, this global maximum point is unique.


Let $z^\star$ be the global maximum of $f(x,\cdot)$, and let $\zeta^\star$ be the global maximum of $f(\theta, \cdot)$.

Then, since $f(x,\cdot)$ is $\alpha$-strongly concave, $\|\nabla_y f(x,z)\| \geq \alpha \|z - z^\star\|$ for all $z \in \mathbb{R}^d$.

Moreover, since $f$ is $L$-smooth, \thetae also have that   $\|\nabla_y f(x,z) - \nabla_y f(\theta,z)\| \leq L\|\theta-x\|$.

Therefore, 

\begin{align} \label{eq_strongly_convex1}
\|\nabla_y f(\theta,z)\| &\geq \|\nabla_y f(x,z) \| - \|\nabla_y f(\theta,z) - \nabla_y f(x,z)\|\\
%
&\geq  \|\nabla_y f(x,z) \|  - L\|\theta-x\|\\
%
&\geq \alpha \|z - z^\star\| - L\|\theta-x\|
\end{align}

Since $\alpha \|z - z^\star\| - L\|\theta-x\|>0$ for any $z \in \mathbb{R}^d$ such that $\|z-z^\star\| > \frac{L}{\alpha}\|\theta-x\|$, \eqref{eq_strongly_convex1} implies that 
%
\begin{equation}
    \|\mathrm{argmax}_{z \in \mathbb{R}^d} f(x,z) -  \mathrm{argmax}_{z \in \mathbb{R}^d} f(\theta,z)\| \leq \frac{L}{\alpha}\|\theta-x\|
\end{equation}

\end{proof}

\begin{lemma}\label{prop_strongly_convex_2}
If $(x,w)\in \mathbb{R}^d\times \mathbb{R}^d$  are such that $\|\nabla_y f(x,w)\| \leq \epsilon$ then $\|w -\mathrm{argmax}_{z \in \mathbb{R}^d} f(x, z) \| \leq \frac{\eps}{\alpha}$.
\end{lemma}



\begin{proof}
Let  $z^\star$ be the unique global maximum point of $f(x,\cdot)$.


Since $f(x, \cdot)$ is $\alpha$-strongly concave, we have that
%
 \begin{align} \label{eq_strongly_convex2}
 \alpha \|w - z^\star\| &\leq \|\nabla_y f(x,w)\|\\
 %
 & \leq \epsilon
\end{align}
%

Therefore, \eqref{eq_strongly_convex2} implies that

\begin{align}
\|w -\mathrm{argmax}_{z \in \mathbb{R}^d} f(x, z) \| = \|w - z^\star\| \leq \frac{\eps}{\alpha}.
\end{align}

\end{proof}



\begin{lemma}\label{prop_strongly_convex_3}
For any $x, \theta \in \mathbb{R}^d$,  $$\|\mathcal{L}_\eps(x,y) - \mathcal{L}_\eps(\theta,y)| \leq L \left(2\frac{\eps}{\alpha} +  \frac{L}{\alpha}\|\theta- x\|\right)$$
\end{lemma}

\begin{proof}

Denote by $\hat{P}_\eps(x,y) \subseteq P_\eps(x,y)$ the collection of endpoints of $\eps$-greedy paths where the endpoint $z$ of the path satisfies $\nabla_y f(x,z) = \epsilon$.
%
Since $f$ is smooth, we have that $\sup_{z\in P_\eps(x,y)} f(x,z) = \sup_{z\in \hat{P}_\eps(x,y)} f(x,z)$ (this is true since, if the endpoint $z$ of an  $\eps$-greedy path does not satisfy $\nabla_y f(x,z) = \epsilon$,  then the $\eps$-greedy path can be extended to achieve a higher value of $f$).

Thus, we have that
%
\begin{align}
    &|\mathcal{L}_\eps(x,y) - \mathcal{L}_\eps(\theta,y)| = |\sup_{z\in P_\eps(x,y)} f(x,z) - \sup_{w\in P_\eps(\theta,y)} f(\theta,w)|\\
    %
     &= |\sup_{z\in \hat{P}_\eps(x,y)} f(x,z) - \sup_{w\in \hat{P}_\eps(\theta,y)} f(\theta,w)|\\
    %
    &\leq \sup_{z\in \hat{P}_\eps(x,y), w\in \hat{P}_\eps(\theta,y)} | f(x,z) - f(\theta,w)|\\
    %
    &\leq \sup_{z\in \hat{P}_\eps(x,y), w\in \hat{P}_\eps(\theta,y)} L \times \|w-z\|\\
    %
    &\leq \sup_{z\in \hat{P}_\eps(x,y), w\in \hat{P}_\eps(\theta,y)} L \times \left(\|w - \mathrm{argmax}_{\zeta \in \mathbb{R}^d} f(\theta,\zeta)\| +  \|\mathrm{argmax}_{\zeta \in \mathbb{R}^d} f(\theta,\zeta)- \mathrm{argmax}_{\zeta \in \mathbb{R}^d} f(x,\zeta)\| + \|\mathrm{argmax}_{\zeta \in \mathbb{R}^d} f(x,\zeta) -z\|\right)\\
    %
    & \stackrel{\textrm{Lemmas \ref{prop_strongly_convex_1}, \ref{prop_strongly_convex_2}}}{\leq} L\times (\frac{\eps}{\alpha} + \frac{L}{\alpha}\|\theta-x\| +\frac{\eps}{\alpha})\\
    %
    &= L\times (2\frac{\eps}{\alpha} + \frac{L}{\alpha}\|\theta-x\|),
\end{align}
%
where the last inequality holds by Proposition \ref{prop_strongly_convex_2} because $\|\nabla_y f(x, z)\| = \eps$ whenever  $z\in \hat{P}_\eps(x,y)$ and $\|\nabla_y f(\theta, w)\| = \eps$ whenever $w\in P_\eps(\theta,y)$.
\end{proof}

\begin{lemma}\label{prop_strongly_convex_4}
For any $x,y \in \mathbb{R}^d$ we have $$|\mathcal{L}_\eps(x,y) - \mathcal{L}_0(x,y)| \leq L \frac{\eps^2}{2 \alpha^2}$$
\end{lemma}

\begin{proof}

\begin{align}
|\mathcal{L}_\eps(x,y) - \mathcal{L}_0(x,y)|  &= |\sup_{z \in \hat{P}(x,y)} f(x,z) - f(x, \mathrm{argmax}_{z\in \mathbb{R}^d} f(x,z)|\\
%
&\leq  \sup_{z \in \hat{P}(x,y)}|f(x,z) - f(x, \mathrm{argmax}_{z\in \mathbb{R}^d} f(x,z))|\\
%
&\leq \sup_{z \in \hat{P}(x,y)} \frac{L}{2}\|z - \mathrm{argmax}_{z\in \mathbb{R}^d} f(x,z)\|^2\\
%
&\stackrel{\textrm{Lemmas  \ref{prop_strongly_convex_2}}}{\leq} \frac{L}{2} (\frac{\eps}{\alpha})^2,
\end{align}
%
where the last inequality holds by Proposition \ref{prop_strongly_convex_2} because $\|\nabla_y f(x, z)\| = \eps$ whenever  $z\in \hat{P}_\eps(x,y)$.

\end{proof}

\begin{lemma}\label{prop_strongly_convex_5}
$\mathcal{L}_0(x^\star, y^\star)$ is differentiable and
%
$$\| \nabla_x f(x^\star, y^\star) - \nabla_x \mathcal{L}_0(x^\star, y^\star) \| \leq L \frac{\eps}{\alpha}$$
\end{lemma}

\begin{proof}

Since $f(x,\cdot)$ is concave, we have that $\mathcal{L}_0(x^\star, y^\star) = \max_{z\in \mathbb{R}^d} f(x^\star, z)$.

Moreover, by strong concavity $f(x^\star, \cdot)$ has a unique maximizer $\mathrm{argmax}_{z\in \mathbb{R}^d} f(x^\star, z)$.

Thus, by Danskin's Theorem \cite{danskin1966theory}, we have that $ \mathcal{L}_0(x^\star, \cdot)$ is differentiable and that 
%
\begin{equation}\label{eq_strongly_convex_3}
    \nabla_x  \mathcal{L}_0(x^\star, y^\star) = \nabla_x f(x^\star, \mathrm{argmax}_{z\in \mathbb{R}^d} f(x^\star, z)).
    \end{equation}

Therefore, since $f$ is $L$-smooth,
%
\begin{align}
    \| \nabla_x f(x^\star, y^\star) - \nabla_x \mathcal{L}_0(x^\star, y^\star) \| &\stackrel{\textrm{Eq.  \ref{eq_strongly_convex_3}}}{=} \| \nabla_x f(x^\star, y^\star) -  \nabla_x f(x^\star, \mathrm{argmax}_{z\in \mathbb{R}^d} f(x^\star, z)) \|\\
    %
&\leq    L \times \|y^\star - \mathrm{argmax}_{z\in \mathbb{R}^d} f(x^\star, z)) \|\\
%
&\leq  L \times \frac{\eps}{\alpha},
\end{align}
%
where the last inequality holds by Lemma \ref{prop_strongly_convex_2} since $\|\nabla_y f(x^\star, y^\star)\| \leq \eps$.

\end{proof}

\begin{proof}[Proof of Theorem \ref{thm_strongly_convex}]

Since $(x^\star, y^\star)$ is an $(\eps, \delta, \omega, Q)$-approximate local equilibrium of $f$, we have that,
%
\begin{equation}
    \|\nabla_y f(x^\star, y^\star)\| \leq \eps
\end{equation}
%
and that, with probability at least $1-\omega$,
%
\begin{equation}
    \mathcal{L}_\eps(x^\star - \Delta, y^\star) \geq f(x^\star, y^\star) - \delta,
\end{equation}
%
where $\Delta \sim Q_{x^\star, y^\star}$.

Thus, since by Assumption \ref{assumption_x_stochastic_gradient} $\mathbb{E}_{\Delta \sim Q_{x,y}}[\Delta] = \mu \nabla_x f(x,y)$ and $\mathbb{E}_{\Delta \sim Q_{x,y}}[\|\Delta -\mu \nabla_x\|^2] \leq \sigma^2$, by Markov's inequality, we have that, with probability at least $1-\2\omega$,
%
\begin{equation}\label{eq_strongly_convex_4}
    \mathcal{L}_\eps(x^\star - \mu \nabla_x f(x^\star, y^\star) + \nu, y^\star) \geq f(x^\star, y^\star) - \delta,
\end{equation}
%
for some $\nu \in \mathbb{R}^d$ such that $\|\nu\|\leq \frac{\sigma}{\sqrt{\omega}}$

Therefore, by plugging in Lemma \ref{prop_strongly_convex_4} to the LHS of  \eqref{eq_strongly_convex_4}  and applying Lemma \ref{prop_strongly_convex_2} together with the fact that $f$ is $L$-smooth to the RHS of  \eqref{eq_strongly_convex_4}, we have that
%
\begin{align}\label{eq_strongly_convex_5}
        \mathcal{L}_0(x^\star - \mu \nabla_x f(x^\star, y^\star) + \nu, y^\star) + L \frac{\eps^2}{2 \alpha^2} \geq \mathcal{L}_0(x^\star, y^\star) - L \frac{\eps}{\alpha}- \delta,
\end{align}
%

Therefore, applying Lemma \ref{prop_strongly_convex_5} to  \eqref{eq_strongly_convex_5} we get that
%
\begin{align}\label{eq_strongly_convex_6}
        \mathcal{L}_0(x^\star - \mu \nabla_x \mathcal{L}_0(x^\star, y^\star) + v, y^\star) + L \frac{\eps^2}{2 \alpha^2} \geq \mathcal{L}_0(x^\star, y^\star) - L \frac{\eps}{\alpha}- \delta,
\end{align}
%
for some $v \in \mathbb{R}^d$ such that $\|v\|\leq L\frac{\eps}{\alpha} + \frac{\sigma}{\sqrt{\omega}}$.

Therefore, plugging in Lemma \ref{prop_strongly_convex_5} to the LHS of \eqref{eq_strongly_convex_6}, we get that
%
\begin{align}\label{eq_strongly_convex_6}
        \mathcal{L}_0(x^\star - \mu \nabla_x \mathcal{L}_0(x^\star, y^\star), y^\star) + L \left(2\frac{\eps}{\alpha} +  \mu \frac{L}{\alpha}(L\frac{\eps}{\alpha} + \frac{\sigma}{\sqrt{\omega}})\right) + L \frac{\eps^2}{2 \alpha^2} \geq \mathcal{L}_0(x^\star, y^\star) - L \frac{\eps}{\alpha}- \delta,
\end{align}
%
since $\|v\|\leq L\frac{\eps}{\alpha} + \frac{\sigma}{\sqrt{\omega}}$.


We also have that
\begin{align}\label{eq_strongly_convex_7}
\mathcal{L}_0(x^\star - \mu \nabla_x \mathcal{L}_0(x^\star, y^\star), y^\star) = \mathcal{L}_0(x^\star, y^\star) -(\nabla_x \mathcal{L}_0(x^\star, y^\star) + u)^\top \mu \nabla_x \mathcal{L}_0(x^\star, y^\star),
\end{align}
%
for some $u \in \mathbb{R}^d$ such that $\|u\| \leq L \| \mu \nabla_x \mathcal{L}_0(x^\star, y^\star)\|$, since $f$ is $L$-smooth.

Therefore \eqref{eq_strongly_convex_7} implies that
%
\begin{align}\label{eq_strongly_convex_8}
\mathcal{L}_0(x^\star - \mu \nabla_x \mathcal{L}_0(x^\star, y^\star), y^\star) \leq \mathcal{L}_0(x^\star, y^\star) - (\mu-\mu^2)\|\nabla_x \mathcal{L}_0(x^\star, y^\star)\|^2,
\end{align}

Plugging \eqref{eq_strongly_convex_8} into \eqref{eq_strongly_convex_6}, we get that (since $0<\mu<1$ implies that $\mu - \mu^2>0$),
%
\begin{align}\label{eq_strongly_convex_9}
        \|\nabla_x \mathcal{L}_0(x^\star, y^\star)\| \leq \frac{1}{\mu-\mu^2}\sqrt{\delta + L \left(2\frac{\eps}{\alpha} + \mu \frac{L}{\alpha}(L\frac{\eps}{\alpha} + \frac{\sigma}{\sqrt{\omega}})\right) + L \frac{\eps^2}{2 \alpha^2} +L \frac{\eps}{\alpha}}
\end{align}

But from \eqref{eq_strongly_convex_3} we have that
%
\begin{equation}\label{eq_strongly_convex_10}
    \nabla_x  \mathcal{L}_0(x^\star, y^\star) = \nabla_x f(x^\star, \mathrm{argmax}_{z\in \mathbb{R}^d} f(x^\star, z)).
    \end{equation}

Thus,
%
\begin{align}\label{eq_strongly_convex_11}
    \|\nabla_x  \mathcal{L}_0(x^\star, y^\star) - \nabla_x  f(x^\star, y^\star)\| &\stackrel{\textrm{Eq.  \ref{eq_strongly_convex_10}}}{=}  \|\nabla_x f(x^\star, \mathrm{argmax}_{z\in \mathbb{R}^d} f(x^\star, z))  - \nabla_x  f(x^\star, y^\star)\|\\
    %
    &\leq L \|y^\star - \mathrm{argmax}_{z\in \mathbb{R}^d} f(x^\star, z)\|\\
    %
 &\stackrel{\textrm{Lemma  \ref{prop_strongly_convex_2}}}{\leq}  L \frac{\eps}{\alpha},
    \end{align}
%
where the first inequality holds since $f$ is $L$-smooth, and the second inequality holds by Lemma  \ref{prop_strongly_convex_2} since $\|\nabla_y f(x^\star, y^\star)\|\leq \eps$.


Plugging in \eqref{eq_strongly_convex_11} into \eqref{eq_strongly_convex_9}, we get
%
\begin{align}\label{eq_strongly_convex_13}
        \|\nabla_x f(x^\star, y^\star)\| \leq \frac{1}{\mu-\mu^2}\sqrt{\delta + L \left(2\frac{\eps}{\alpha} + \mu \frac{L}{\alpha}(L\frac{\eps}{\alpha} + \frac{\sigma}{\sqrt{\omega}})\right) + L \frac{\eps^2}{2 \alpha^2} +L \frac{\eps}{\alpha}} +  L \frac{\eps}{\alpha}.
\end{align}

Now, since $f(\cdot, y^\star)$ is $\alpha$-strongly convex, by Lemma \ref{prop_strongly_convex_2} (applied to $-f$ instead of $f$), we have
%
\begin{align} \label{eq_strongly_convex_14}
    \|x^\star - \mathrm{argmin}_{\theta \in \mathbb{R}^d} f(\theta, y^\star)\|  \leq \frac{\|\nabla_x f(x^\star, y^\star)\|}{\alpha}
\end{align}

Since $f$ is $L$-smooth, \eqref{eq_strongly_convex_14} implies that
%
\begin{align} \label{eq_strongly_convex_15}
    f(x^\star,y^\star) - \min_{\theta \in \mathbb{R}^d} f(\theta, y^\star) &\leq  L \times  \frac{1}{2}\|x^\star - \mathrm{argmin}_{\theta \in \mathbb{R}^d} f(\theta, y^\star)\|^2\\
    %
    &\stackrel{\textrm{Eq. \ref{eq_strongly_convex_14}}}{\leq}\frac{L}{2} \times \left(\frac{\|\nabla_x f(x^\star, y^\star)\|}{\alpha}\right)^2
\end{align}



Moreover, since $f(x^\star, \cdot)$ is $\alpha$-strongly concave and $\nabla_y f(x^\star, y^\star)$ we have  by Lemma \ref{prop_strongly_convex_2} that 
%
 \begin{align} \label{eq_strongly_convex_16}
 %
 \|y^\star -\mathrm{argmax}_{z \in \mathbb{R}^d} f(x^\star, z) \| \leq \frac{\eps}{\alpha}.
 \end{align}
 %
 Since $f$ is $L$-smooth, \eqref{eq_strongly_convex_16} implies that
 %
 \begin{align} \label{eq_strongly_convex_17}
    \max_{z \in \mathbb{R}^d} f(x^\star, z) - f(x^\star,y^\star) &\leq  L \times  \frac{1}{2}\|y^\star - \mathrm{argmax}_{z \in \mathbb{R}^d} f(x^\star, z)\|^2\\
    %
    &\stackrel{\textrm{Eq. \ref{eq_strongly_convex_16}}}{\leq}\frac{L}{2} \times \left(\frac{\eps}{\alpha}\right)^2
\end{align}

Thus, adding \eqref{eq_strongly_convex_15} to \eqref{eq_strongly_convex_17}, and plugging in \eqref{eq_strongly_convex_13}, we get that
%
%
\begin{align} \label{eq_strongly_convex_18}
     &\max_{z \in \mathbb{R}^d} f(x^\star, z)  - \min_{\theta \in \mathbb{R}^d} f(\theta, y^\star) \leq  L \times  \frac{1}{2}\|x^\star - \mathrm{argmin}_{\theta \in \mathbb{R}^d} f(\theta, y^\star)\|^2 + \\
    %
    &\stackrel{\textrm{Eq. \ref{eq_strongly_convex_14}}}{\leq}\frac{L}{2} \times \left(\frac{\|\nabla_x f(x^\star, y^\star)\|}{\alpha}\right)^2 + \frac{L}{2} \times \left(\frac{\eps}{\alpha}\right)^2\\
    %
    & \stackrel{\textrm{Eq. \ref{eq_strongly_convex_13}}}{\leq}
    %
    \frac{L\eps^2}{2\alpha^2} + 
    %
    \frac{L}{2\alpha^2}
   \left(\frac{1}{\mu-\mu^2}\sqrt{\delta + L \left(2\frac{\eps}{\alpha} + \mu \frac{L}{\alpha}(L\frac{\eps}{\alpha} + \frac{\sigma}{\sqrt{\omega}})\right) + L \frac{\eps^2}{2 \alpha^2} +L \frac{\eps}{\alpha}} +  L \frac{\eps}{\alpha}\right)^2
\end{align}

Since $\mu= \frac{1}{L}$, we get that

\begin{align} \label{eq_strongly_convex_19}
     &\max_{z \in \mathbb{R}^d} f(x^\star, z)  - \min_{\theta \in \mathbb{R}^d} f(\theta, y^\star) \leq
    %
    \frac{L\eps^2}{2\alpha^2} + 
    %
    \frac{L}{2\alpha^2}
   \left(\frac{1}{\mu-\mu^2}\sqrt{\delta + L \left(2\frac{\eps}{\alpha} + \mu \frac{L}{\alpha}(L\frac{\eps}{\alpha} + \frac{\sigma}{\sqrt{\omega}})\right) + L \frac{\eps^2}{2 \alpha^2} +L \frac{\eps}{\alpha}} +  L \frac{\eps}{\alpha}\right)^2\\
   %
   &=\frac{L\eps^2}{2\alpha^2} + 
    %
    \frac{L^3}{2\alpha^2}
   \left(\sqrt{\delta + L \left(2\frac{\eps}{\alpha} + \mu \frac{L}{\alpha}(L\frac{\eps}{\alpha} + \frac{\sigma}{\sqrt{\omega}})\right) + L \frac{\eps^2}{2 \alpha^2} +L \frac{\eps}{\alpha}} +  L \frac{\eps}{\alpha}\right)^2
\end{align}

\end{proof}


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
